Unasssuming View-Size Estimation Techniques in OLAP

Even if storage was infinite, a data warehouse could not materialize all possible views due to the running time and update requirements. Therefore, it is necessary to estimate quickly, accurately, and reliably the size of views. Many available techniques make particular statistical assumptions and their error can be quite large. Unassuming techniques exist, but typically assume we have independent hashing for which there is no known practical implementation. We adapt an unassuming estimator due to Gibbons and Tirthapura: its theoretical bounds do not make unpractical assumptions. We compare this technique experimentally with stochastic probabilistic counting, LogLog probabilistic counting, and multifractal statistical models. Our experiments show that we can reliably and accurately (within 10%, 19 times out 20) estimate view sizes over large data sets (1.5 GB) within minutes, using almost no memory. However, only Gibbons-Tirthapura provides universally tight estimates irrespective of the size of the view. For large views, probabilistic counting has a small edge in accuracy, whereas the competitive sampling-based method (multifractal) we tested is an order of magnitude faster but can sometimes provide poor estimates (relative error of 100%). In our tests, LogLog probabilistic counting is not competitive. Experimental validation on the US Census 1990 data set and on the Transaction Processing Performance (TPC H) data set is provided.

==> abstract.tex <==
\fontsize{9}{11}\selectfont Even if storage was infinite, a data warehouse
could not materialize all possible views due to the running time and update
requirements. Therefore, it is necessary to estimate quickly, accurately, and reliably the
size of views. Many available techniques make particular statistical
assumptions and their error can be quite large. Unassuming techniques exist,
but typically assume we have independent hashing for which there is no known
practical implementation. We adapt an unassuming estimator due to Gibbons and
Tirthapura: its theoretical bounds do not
make unpractical assumptions.
We compare this technique experimentally with stochastic
probabilistic counting, \textsc{LogLog} probabilistic counting, and
multifractal statistical models. %For \textsc{group by} aggregations on $k$~dimensions,
%we use $k$-wise independent hashing.
% Out of all these techniques, 
 Our experiments show that
we can reliably and accurately (within 10\%, 19 times out 20) estimate view sizes over 
large data sets (1.5\,GB) within minutes, using almost no  memory.
However, only
\textsc{Gibbons-Tirthapura} provides universally tight estimates irrespective of the
size of the view. For large views, probabilistic counting has a small edge in accuracy,
whereas the competitive sampling-based method (multifractal)
we tested is an order of magnitude faster but can sometimes provide poor
estimates (relative error of 100\%). In our tests, \textsc{LogLog} probabilistic counting
is not competitive.
Experimental validation on the US Census 1990 data set and on the  Transaction Processing Performance (TPC~H) data set is provided.


==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont{}
  Kamel Aouiche and Daniel Lemire\\
  \fontsize{9}{11}\selectfont{}
  \textit{LICEF, University of Quebec at Montreal, 100 Sherbrooke West, Montreal, Canada}\\
  \fontsize{9}{11}\selectfont{}
  \textit{kamel.aouiche@gmail.com, lemire@acm.org}%\\[12pt] 
%\vspace{-100cm}
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont probabilistic estimation, skewed distributions, sampling, hashing


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{
\uppercase{Unasssuming View-Size Estimation Techniques in OLAP}
% \uppercase{Authors' Instructions}\\
% % The Subtitle should have initial letters capitalized
 \fontsize{13}{15}\selectfont \textit{An Experimental Comparison
}
}

